DARTH: Holistic Test-time Adaptation for Multiple Object Tracking

Multiple object tracking (MOT) is a fundamental component of perception systems for autonomous driving, and its robustness to unseen conditions is a requirement to avoid life-critical failures. Despite the urge of safety in driving systems, no solution to the MOT adaptation problem to domain shift in test-time conditions has ever been proposed. However, the nature of a MOT system is manifold - requiring object detection and instance association - and adapting all its components is non-trivial. In this paper, we analyze the effect of domain shift on appearance-based trackers, and introduce DARTH, a holistic test-time adaptation framework for MOT. We propose a detection consistency formulation to adapt object detection in a self-supervised fashion, while adapting the instance appearance representations via our novel patch contrastive loss. We evaluate our method on a variety of domain shifts - including sim-to-real, outdoor-to-indoor, indoor-to-outdoor - and substantially improve the source model performance on all metrics. Code: https://github.com/mattiasegu/darth.

==> figures/method_schematic.tex <==
\begin{figure}[!ht]
  \centering
  \resizebox{\linewidth}{!}{
%   \includegraphics[trim={0.0cm 5.2cm 2.5cm 0},clip]
  \includegraphics{images/method_schematic.pdf}
  }
  \caption{Schematic representation on the target domain of DARTH, our test-time adaptation method for \ac{mot}. Our patch contrastive loss $\mathcal{L}_{\text{PCL}}$ between the siamese student's detection embeddings adapts instance association while learning local target representations. Our detection consistency loss $\mathcal{L}_{\text{DC}}$ enforces consistency to photometric changes while fostering good global target representations. The \ac{ema} updates to the teacher gradually improve the detection targets for our consistency loss by benefiting from the adapted student representations. $\phi_T$, $\phi_S$, and $\phi_C$ are the image transformations described in \Cref{ssec:darth_overview} to generate the teacher, student, and contrastive views. `//' = stop gradient. \mattia{FINAL. Should this be the teaser or the teaser should introduce the domain adaptation problem for MOT?} \bernt{good question\dots, I suppose we need this figure somewhere and here it can work imho - even though it is a bit tedious to go through it. Not sure what you have in mind to `illustrate the DA problem for MOT'? I suppose the general DA-problem is clear?  -- an alternative could be some qualitative result before and after test-time adaption that looks striking / convincing? - this could serve both the DA-problem illustration as well as showing some initial qualitative results?} \mattia{yes, I will make a draft showing tracking results before and after TTA}
  \tao{Imho, maybe this framework figure will be more clear and more attracting if some visualizations are provided for the ``Input Image'' and three augmented views, if space allowed. } \mattia{makes sense, I will make a draft and see if it is feasible in the limited space we have. same for figure 2 where I can try to also replace the input image block with the corresponding clean input image}
  } \label{fig:method_schematic}
\end{figure}



==> figures/patch_contrastive_learning.tex <==
\begin{figure*}
  \centering
  \resizebox{\textwidth}{!}{
  \includegraphics{images/patch_contrastive_learning.pdf}
  }
  \caption{We here illustrate our novel patch contrastive formulation (\Cref{ssec:darth_patch_contrastive_learning}). First, we identify object regions by applying the teacher detector on the input image and filtering the detections based on their confidence. We then apply on the input image and detected bounding boxes the transformations $\hat{\phi}_S$ and $\phi_C$ to generate the student and constrastive view, deriving association pseudo-labels by considering a match as positive when proposed regions (white) on different views match to a same teacher detection (identified by the same color across both views). Finally, we apply a multi-positive patch contrastive loss on the projections of the proposed regions obtained via the student embedding head. We here show an example of positive (green) and negative (red) matches for one of the student-view proposed regions.
  } \label{fig:patch_contrastive_learning}
\end{figure*}



==> sections/0_abstract_old.tex <==
\begin{abstract}
% what is MOT and why it is important to adapt
Multiple object tracking (MOT) is a fundamental component of perception systems for autonomous driving, and its robustness to unseen conditions is a requirement to avoid life-critical failures.
%
Despite the urge of safety in driving systems, no solution to the MOT adaptation problem to domain shift in test-time conditions has ever been proposed.
% tracking is a system with multiple components --> holistic adaptation
However, the nature of a MOT system is manifold - requiring object detection
, its consistency through time, 
and instance association - and adapting all its components is non-trivial.
% method
In this paper, we introduce DARTH, a holistic test-time adaptation framework for multiple object tracking.
%
We propose a detection consistency formulation to adapt object detection in a self-supervised fashion and enforce its robustness to photometric changes, while learning discriminative local representations and adapting instance association to the target domain via our novel patch contrastive loss. 
%
We evaluate our method on a variety of domain shifts - including sim-to-real, outdoor-to-indoor, indoor-to-outdoor, and contextual shifts - and substantially improve the source model performance on all evaluated metrics.
%
\end{abstract}

==> sections/1_introduction_old.tex <==
\section{Introduction}
%
\Ac{mot} represents a cornerstone of modern perception systems for challenging computer vision applications, such as autonomous driving~\cite{ess2010object}, video surveillance~\cite{elhoseny2020multi}, behavior analysis~\cite{hu2004survey}, and augmented reality~\cite{park2008multiple}.
%
Laying the ground for safety-critical downstream perception and planning tasks - \eg obstacle avoidance, motion estimation, prediction of vehicles and pedestrians intentions, and the consequent path planning - the robustness of \ac{mot} to diverse conditions is of uttermost importance.
 
%  \bernt{detail: I am not a fan of empasizing  e.g., i.e. using e.g. italic style - why is this so important and should stand out? thus I would prefer not using the standard shortcuts `\eg', `\ie', etc.} 
 
However, domain shift~\cite{khosla2012undoing} could result in life-threatening failures of \ac{mot} pipelines, due to the perception system's inability to understand previously unseen environments and provide meaningful signals for downstream planning.
%
% However, domain shift~\cite{khosla2012undoing} could result in potentially life-threatening failures of \ac{mot}-based pipelines, due to the perception system's inability to understand and interact with previously unseen environments.
% \bernt{by definition a perception system is not interacting imho - thus I would rephrase: `perception system's inability to understand previously unseen environments' -- if you want to add the interaction I would suggest to talk about the `autonomous system' and not the `perception system' -- but that seems somewhat too far reaching as an argument imho} 
%
To the best of our knowledge, despite the urge of addressing domain adaptation for \ac{mot} to enable safer driving and video analysis, no solution has ever been proposed.
% \bernt{should we make this slightly less pushy? something like: `... to the best of our knowledge, no solution has ever been proposed'?}

%%%%%%%%%%%%%%%%%%%%%%
% TEASER/METHOD FIGURE
%%%%%%%%%%%%%%%%%%%%%%
% \input{figures/method_schematic}
\input{figures/teaser}
%%%%%%%%%%%%%%%%%%%%%%
The domain shift problem has been traditionally tackled in deep learning with \ac{uda} techniques~\cite{wilson2020survey}, aligning the deep distribution of a labeled source domain and an unlabeled target domain~\cite{tzeng2017adversarial,li2016revisiting,tzeng2014deep,segu2020batch}. 
% by means of adversarial learning~\cite{tzeng2017adversarial}, adaptive normalization~\cite{li2016revisiting} or discrepancy minimization~\cite{tzeng2014deep,long2015learning}.
%
However, assuming the availability of target data at training time hinders the practicality of such techniques, as the real-world continuously mutates and not all possible test scenarios can be known in advance.

% Discuss TTA
\Ac{tta} offers a more realistic solution to domain shift by adapting a pre-trained model to any unlabeled target domain in absence of the original source domain.
%
Current \ac{tta} techniques are tailored to classification tasks~\cite{wang2020tent,chen2022contrastive,wang2022continual,mirza2022norm} or require altering the source training procedure~\cite{sun2020test,liu2021ttt++,noroozi2016unsupervised}, and while they have been shown to work well in simple scenarios, they struggle in more complex ones~\cite{liu2021ttt++}.
%
Recent work further investigates \ac{tta} for object detection, relying on detection pseudo labels~\cite{li2021free} or image-level representation learning~\cite{sinha2022test}.
%
Although modern \ac{mot} methods rely on the tracking-by-detection paradigm, solving \ac{tta} for detection is not sufficient, as instance association and detection consistency to view changes also play a crucial role in tracking. 
%
This is observed in \Cref{tab:sota_pedestrians_to_bdd}, where SFOD~\cite{li2021free} - a \ac{tta} method for object detection - improves the baseline DetA while worsening tracking related metrics.
% \bernt{do you have evidence that detection adaptation is not sufficient later in the experiments? If yes, it would be great to already forward reference to the section/table} \mattia{yes, SFOD only adapts detection and often worsens association}

To this end, we introduce a holistic test-time adaptation framework that addresses the manifold nature of \ac{mot} (\Cref{fig:method_schematic}).
% \mattia{maybe expand here or in previous sentence that MOT compared to detection has to face three problems: detection, detection consistency, and data association}
% detection consistency
We propose a detection consistency formulation to adapt object detection in a self-supervised fashion and enforce its robustness to photometric changes, since tracking benefits from consistency of detection results in adjacent frames.
% pcl
Moreover, we adapt instance association and learn meaningful local target representations by introducing a patch contrastive loss, which enforces self-matching of detected instances under differently augmented views of the same image.
% ema
Finally, we update the teacher as an \ac{ema} of the student model to benefit from the adapted student representations and gradually improve the detection targets for our consistency loss.

We name DARTH our test-time Domain Adaptation method for Recovering multiple object Tracking Holistically.
%
To the best of our knowledge, our proposal is the first solution to the domain adaptation problem for \ac{mot}.
%
We evaluate DARTH on a variety of domain shifts across the driving datasets SHIFT~\cite{sun2022shift} and BDD100K~\cite{yu2018bdd100k}, and the pedestrian datasets MOT17~\cite{milan2016mot16} and DanceTrack~\cite{sun2022dancetrack}, showing substantial improvements over the source model performance on all the evaluated metrics and settings.
%

We summarize our contributions: (i) we introduce the first solution to \ac{tta} for \ac{mot}; (ii) we propose a detection consistency formulation to adapt object detection and enforce its consistency to photometric changes; (iii) we introduce a patch contrastive approach to adapt data association.
% \bernt{I tend to prefer a clear list of contributions so that the reviewer/reader knows what exactly we are claiming as our key contributions -- that should be possible -- right?} \mattia{yes, need to do it after sharpening the intro}


==> tables/rebuttal/multiframe.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\footnotesize
% \setlength{\tabcolsep}{3.7pt}
\begin{tabular}{@{}lccccc@{}}
\toprule
Method   & DetA          & MOTA          & HOTA          & IDF1          & AssA          \\ \midrule
No Adap. & 52.4          & 57.2          & 21.5          & 19.5          & 9.0           \\
% CoTTA &           &           &           &           &            \\
DARTH    & 57.2          & 70.1          & 31.6          & 32.8          & 17.7          \\
DARTH-v  & \textbf{63.0} & \textbf{74.0} & \textbf{39.3} & \textbf{40.2} & \textbf{24.8} \\ \bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{Comparison on MOT17 $\rightarrow$ DT of No Adap., CoTTA, single-frame DARTH, multi-frame DARTH-v leveraging gt IDs.}
\label{tab:multi-frame}
\vspace{-1.8em}
\end{table}

==> tables/sota/bdd_weather_average.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\footnotesize
\setlength{\tabcolsep}{3.7pt}
\begin{tabular}{@{}lccccccc@{}}
\toprule
Method                 & Source                   & Target                   & DetA         & MOTA          & HOTA          & IDF1          & AssA          \\ \midrule
No Adap.               & \multirow{4}{*}{daytime} & \multirow{4}{*}{night}   & \textbf{4.7} & -3.7          & 12.2          & 30.6          & 34.8          \\
Tent~\cite{wang2020tent} &                                                                          &                          &           &             &           &           &           \\
SFOD~\cite{li2021free} &                          &                          & \textbf{4.7} & -2.2          & \textbf{12.6} & \textbf{32.0}   & \textbf{37.8} \\
Ours                   &                          &                          & \textbf{4.7} & \textbf{6.6}  & \textbf{12.6} & 31.9          & 37.7          \\ \midrule 
\rowcolor[HTML]{EFEFEF}Oracle                 &   night                       &  night                        & 5.9          & 18.3          & 15.1          & 39.4          & 41.2          \\ \midrule
No Adap.               & \multirow{4}{*}{night}   & \multirow{4}{*}{daytime} & 4.0            & 11.0            & 11.7          & 29.7          & 37.7          \\
Tent~\cite{wang2020tent} &                                                                          &                          &           &             &           &           &           \\
SFOD~\cite{li2021free} &                          &                          & 3.9          & 14.0            & 11.4          & 29.4          & 35.3          \\
Ours                   &                          &                          & \textbf{4.1} & \textbf{14.2} & \textbf{12.0}   & \textbf{30.9} & \textbf{37.9} \\ \midrule 
\rowcolor[HTML]{EFEFEF}Oracle                 &  daytime                        &  daytime                        & 6.6          & 19.1          & 17.5          & 45.4          & 48.0          \\ \bottomrule
\end{tabular}
\caption{\textbf{State of the art on BDD100K time-of-day shifts (Average).} We benchmark our method (Ours) against baseline test-time adaptation methods for adapting a \ac{mot} model across clear-daytime (daytime) and clear-night (night) conditions on the BDD100K dataset. For each metric we report its average across all object categories.}
\label{tab:sota_bdd_weather_average}
\end{table}

==> tables/sota/bdd_weather_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\footnotesize
\setlength{\tabcolsep}{3.7pt}
\begin{tabular}{@{}lccccccc@{}}
\toprule
Method                 & Source                   & Target                   & DetA          & MOTA          & HOTA          & IDF1          & AssA          \\ \midrule
No Adap.               & \multirow{3}{*}{daytime} & \multirow{3}{*}{night}   & 12.8          & 37.6          & 26.4          & 57.7          & 55.6          \\
SFOD~\cite{li2021free} &                          &                          & 12.7          & \textbf{42.5} & 26.5          & 59.2          & 56.2          \\
Ours                   &                          &                          & \textbf{13.2} & 39.4          & \textbf{27.2} & \textbf{59.5} & \textbf{56.9} \\ \midrule 
\rowcolor[HTML]{EFEFEF}Oracle                 & night                         & night                          & 14.8          & 52.4          & 30.4          & 67.3          & 63.2          \\ \midrule
No Adap.               & \multirow{3}{*}{night}   & \multirow{3}{*}{daytime} & 9.0             & 38.0            & 22.4          & 54.8          & 56.3          \\
SFOD~\cite{li2021free} &                          &                          & 8.9           & \textbf{40.4} & 22.5          & 55.7          & \textbf{57.1} \\
Ours                   &                          &                          & \textbf{9.2}  & 39.4          & \textbf{22.7} & \textbf{55.9} & 56.9          \\ \midrule
\rowcolor[HTML]{EFEFEF}Oracle                 &  daytime                        &  daytime                        & 11.4          & 52.4          & 26.6          & 65.6          & 62.4          \\ \bottomrule
\end{tabular}
\caption{\textbf{State of the art on BDD100K time-of-day shifts (Overall).} We benchmark our method (Ours) against baseline test-time adaptation methods for adapting a \ac{mot} model across clear-daytime (daytime) and clear-night (night) conditions on the BDD100K dataset. For each metric we report the overall result across all categories.}
\label{tab:sota_bdd_weather_overall}
\end{table}

==> tables/sota/domain_shift_mot_bytetrack.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llccccc@{}}
\toprule
Source                         & Target                             & DetA                         & MOTA                         & HOTA                         & IDF1                         & AssA                         \\ \midrule
                               & \cellcolor[HTML]{E0FCE0}SHIFT      & \cellcolor[HTML]{E0FCE0}46.7 & \cellcolor[HTML]{E0FCE0}46.6 & \cellcolor[HTML]{E0FCE0}55.1 & \cellcolor[HTML]{E0FCE0}60.6 & \cellcolor[HTML]{E0FCE0}65.7 \\
\multirow{-2}{*}{SHIFT}        & BDD100K                            & 11.8                         & -70.5                        & 15.2                         & 14.8                         & 23.4                         \\ \midrule
                               & \cellcolor[HTML]{E0FCE0}MOT17      & \cellcolor[HTML]{E0FCE0}56.7 & \cellcolor[HTML]{E0FCE0}65.8 & \cellcolor[HTML]{E0FCE0}57.5 & \cellcolor[HTML]{E0FCE0}68.9 & \cellcolor[HTML]{E0FCE0}58.9 \\
                               & DanceTrack                         & 52.2                         & 62.2                         & 31.6                         & 35.5                         & 19.4                         \\
\multirow{-3}{*}{MOT17}        & BDD100K                            & 22.6                         & -12.0                        & 21.3                         & 22.4                         & 20.5                         \\ \midrule
                               & \cellcolor[HTML]{E0FCE0}MOT17      & \cellcolor[HTML]{E0FCE0}60.0 & \cellcolor[HTML]{E0FCE0}70.3 & \cellcolor[HTML]{E0FCE0}58.8 & \cellcolor[HTML]{E0FCE0}71.4 & \cellcolor[HTML]{E0FCE0}58.1 \\
                               & DanceTrack                         & 61.1                         & 75.2                         & 36.1                         & 38.9                         & 21.5                         \\
\multirow{-3}{*}{MOT17 (+ CH)} & BDD100K                            & 32.9                         & 8.2                          & 27.9                         & 30.4                         & 24.0                         \\ \midrule
                               & \cellcolor[HTML]{E0FCE0}DanceTrack & \cellcolor[HTML]{E0FCE0}65.9 & \cellcolor[HTML]{E0FCE0}77.8 & \cellcolor[HTML]{E0FCE0}40.4 & \cellcolor[HTML]{E0FCE0}41.5 & \cellcolor[HTML]{E0FCE0}25.0 \\
                               & MOT17                              & 25.3                         & 21.6                         & 34.4                         & 38.2                         & 47.3                         \\
\multirow{-3}{*}{DanceTrack}   & BDD100K                            & 7.6                          & -19.2                        & 13.1                         & 10.0                         & 22.9                         \\ \midrule
                               & \cellcolor[HTML]{E0FCE0}BDD100K    & \cellcolor[HTML]{E0FCE0}35.8 & \cellcolor[HTML]{E0FCE0}9.4  & \cellcolor[HTML]{E0FCE0}29.1 & \cellcolor[HTML]{E0FCE0}31.9 & \cellcolor[HTML]{E0FCE0}24.0 \\
                               & MOT17                              & 31.0                         & 29.5                         & 36.3                         & 43.8                         & 43.2                         \\
\multirow{-3}{*}{BDD100K}      & DanceTrack                         & 43.7                         & 44.6                         & 25.2                         & 27.1                         & 14.7                         \\ \bottomrule
\end{tabular}
\caption{\textbf{Domain shift in \ac{mot} (ByteTrack~\cite{zhang2022bytetrack}).} We assess the impact of domain shift on the performance of a ByteTrack model. Highlighted in green is the performance on the source domain. For the ${\text{SHIFT} \rightarrow \text{BDD100K}}$ metrics we report their average across all object categories. For all other experiments, only the pedestrian category is considered. CH is short for CrowdHuman.}
\label{tab:summary_domain_shift_bytetrack}
\end{table}
